RITA: a Study on Scaling Up Generative Protein Sequence Models

In this work we introduce RITA: a suite of autoregressive generative models for protein sequences, with up to 1.2 billion parameters, trained on over 280 million protein sequences belonging to the UniRef-100 database. Such generative models hold the promise of greatly accelerating protein design. We conduct the first systematic study of how capabilities evolve with model size for autoregressive transformers in the protein domain: we evaluate RITA models in next amino acid prediction, zero-shot fitness, and enzyme function prediction, showing benefits from increased scale. We release the RITA models openly, to the benefit of the research community.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> results_table_first_submission.tex <==
\iftrue
\begin{table*}[t]
\caption{\textbf{Fitness evaluation:} We compute the Spearman's rank correlation between the fitness value measured experimentally and the predicted fitness value across 32 proteins, and report the average values. RITA models approach the performance of specialized models with increasing parameter count. Baselines results are based on a single seed. Results provided in full in Table~\ref{tab:full_fitness}. Best performance is in \textbf{bold}.}
\label{tab:fitness}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{lcccc ccc ccc}
\toprule
& \multicolumn{4}{c}{RITA}& \multicolumn{3}{c}{Baselines} \\

& Small & Medium & Large & XLarge &  ESM-1v & MSA Transformer & EVE \\
\midrule
AVG Fitness & 0.393& 0.450& 0.455& 0.460 & 0.474 & 0.478 &  \textbf{0.520}\\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table*}
\else
\begin{table*}[t]
\caption{\textbf{Fitness evaluation:} We compute the spearman correlation between experimentally measured fitness values and the predicted values across 32 proteins and report the average values. For the baselines both single model correlation and the ensembled correlation is reported. We see that results for our models starts to approach specialized models as size increases. Results are obtained with a single seed and provided in full in Table~\ref{tab:full_fitness}}
\label{tab:fitness}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{lcccc ccc ccc}
\toprule
& \multicolumn{4}{c}{RITA}& \multicolumn{3}{c}{Baselines} &  \multicolumn{3}{c}{Baselines + Ensemble}\\

& Small & Medium & Large & XLarge &  ESM-1v & MSA & EVE & ESM-1v & MSA Transformer & EVE \\
\midrule
AVG Fitness & 0.3925& 0.4497& 0.4547& 0.4595& 0.4739& 0.4780 & 0.5197 & 0.5091& 0.4718& \textbf{0.5256}\\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table*}
\fi

\begin{table}[h]
\caption{\textbf{Fitness evaluation:} The Spearman correlation between experimentally measured fitness values for different proteins and the value predicted by the models. We exclude \texttt{BRCA1\_HUMAN}, \texttt{POLG\_HCVJF}, and \texttt{UBE4B\_MOUSE} from the aggregation, since they do not fit in the context length that our model was trained on, and rotary embeddings do not extrapolate well. }
\begin{center}
\begin{tiny}
\begin{tabular}{lccccccc}
\toprule
& \multicolumn{4}{c}{RITA}& \multicolumn{3}{c}{Baselines} \\
                                                 & \multicolumn{1}{c}{S} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{L} & \multicolumn{1}{c}{XL} & \multicolumn{1}{l}{ESM-1v} & \multicolumn{1}{l}{MSA\_transformer} & \multicolumn{1}{l}{EVE} \\
\midrule
\texttt{AMIE\_PSEAE\_Wrenbeck\_2017}                      & 0.49                  & 0.52                  & 0.53                  & 0.56                   & 0.61                             & 0.61                                        & 0.56                           \\
\texttt{B3VI55\_LIPST\_Klesmith\_2015}                    & 0.28                  & 0.39                  & 0.43                  & 0.45                   & 0.48                             & 0.53                                        & 0.44                           \\
\texttt{A0A192B1T2\_9HIV1\_Haddox\_2018}                  & 0.49                  & 0.50                  & 0.50                  & 0.50                   & 0.49                             & 0.51                                        & 0.51                           \\
\texttt{Q2N0S5\_9HIV1\_Haddox\_2018}                      & 0.51                  & 0.42                  & 0.40                  & 0.35                   & 0.5                              & 0.49                                      & 0.5                            \\
\texttt{Q59976\_STRSQ\_Romero\_2015}                      & 0.58                  & 0.64                  & 0.64                  & 0.65                   & 0.51                             & 0.67                                        & 0.65                           \\
\texttt{BLAT\_ECOLX\_Firnberg\_2014}                      & 0.61                  & 0.61                  & 0.59                  & 0.56                   & 0.68                             & 0.74                                        & 0.74                           \\
\texttt{BLAT\_ECOLX\_Deng\_2012}                          & 0.44                  & 0.40                  & 0.42                  & 0.40                   & 0.53                             & 0.56                                        & 0.51                           \\
\texttt{BLAT\_ECOLX\_Stiffler\_2015}                      & 0.61                  & 0.62                  & 0.58                  & 0.57                   & 0.69                             & 0.73                                        & 0.74                           \\
\texttt{BLAT\_ECOLX\_Jacquier\_2013}                      & 0.60                  & 0.59                  & 0.58                  & 0.56                   & 0.68                             & 0.7                                         & 0.74                           \\
\texttt{BRCA1\_HUMAN\_Findlay\_2018}                      & 0.15                  & -0.15                 & -0.19                 & 0.07                   & 0.44                             & 0.4                                         & 0.32                           \\
\texttt{CALM1\_HUMAN\_Weile\_2017}                        & 0.19                  & 0.25                  & 0.26                  & 0.27                   & 0.25                             & 0.25                                        & 0.24                           \\
\texttt{DLG4\_RAT\_McLaughlin\_2012}                      & 0.38                  & 0.39                  & 0.38                  & 0.37                   & 0.56                             & 0.51                                        & 0.52                           \\
\texttt{GAL4\_YEAST\_Kitzman\_2015}                       & 0.29                  & 0.35                  & 0.36                  & 0.35                   & 0.44                             & 0.58                                        & 0.51                           \\
\texttt{A0A2Z5U3Z0\_9INFA\_Doud\_2016}                    & 0.46                  & 0.53                  & 0.52                  & 0.54                   & 0.51                             & 0.16                                        & 0.53                           \\
\texttt{HSP82\_YEAST\_Mishra\_2016}                       & 0.49                  & 0.50                  & 0.49                  & 0.53                   & 0.57                             & 0.48                                        & 0.54                           \\
\texttt{IF1\_ECOLI\_Kelsic\_2016}                         & 0.36                  & 0.46                  & 0.38                  & 0.42                   & 0.54                             & 0.23                                        & 0.52                           \\
\texttt{KKA2\_KLEPN\_Melnikov\_2014}                      & 0.30                  & 0.43                  & 0.54                  & 0.56                   & 0.61                             & 0.58                                        & 0.6                            \\
\texttt{MK01\_HUMAN\_Brenan\_2016}                        & 0.22                  & 0.13                  & 0.10                  & 0.05                   & 0.18                             & 0.15                                        & 0.25                           \\
\texttt{MTH3\_HAEAE\_Rockah-Shmuel}\_2015                 & 0.36                  & 0.49                  & 0.63                  & 0.68                   & 0.7                              & 0.69                                        & 0.71                           \\
\texttt{PABP\_YEAST\_Melamed\_2013}                       & 0.59                  & 0.64                  & 0.66                  & 0.68                   & 0.66                             & 0.67                                        & 0.62                           \\
\texttt{PA\_I34A1\_Wu\_2015}                              & 0.46                  & 0.49                  & 0.53                  & 0.54                   & 0.055                            & 0.38                                        & 0.54                           \\
\texttt{POLG\_HCVJF\_Qi\_2014}                            & 0.40                  & 0.12                  & 0.47                  & 0.44                   & 0.61                             & 0.6                                         & 0.61                           \\
\texttt{RASH\_HUMAN\_Bandaru\_2017}                       & 0.44                  & 0.42                  & 0.42                  & 0.40                   & 0.36                             & 0.42                                        & 0.45                           \\
\texttt{RL401\_YEAST\_Roscoe\_2013}                       & 0.42                  & 0.58                  & 0.56                  & 0.49                   & 0.31                             & 0.43                                        & 0.42                           \\
\texttt{RL401\_YEAST\_Roscoe\_2014}                       & 0.35                  & 0.45                  & 0.42                  & 0.39                   & 0.25                             & 0.36                                        & 0.4                            \\
\texttt{RL401\_YEAST\_Mavor\_2016}                        & 0.38                  & 0.53                  & 0.48                  & 0.43                   & 0.3                              & 0.38                                        & 0.36                           \\
\texttt{SUMO1\_HUMAN\_Weile\_2017}                        & 0.22                  & 0.37                  & 0.41                  & 0.39                   & 0.43                             & 0.42                                        & 0.53                           \\
\texttt{TRPC\_SACS2\_Chan\_2017}                          & 0.43                  & 0.56                  & 0.50                  & 0.57                   & 0.61                             & 0.63                                        & 0.58                           \\
\texttt{TRPC\_THEMA\_Chan\_2017}                          & 0.33                  & 0.39                  & 0.39                  & 0.45                   & 0.47                             & 0.47                                        & 0.42                           \\
\texttt{P84126\_THETH\_Chan\_2017}                        & 0.41                  & 0.51                  & 0.48                  & 0.55                   & 0.55                             & 0.63                                        & 0.57                           \\
\texttt{TPK1\_HUMAN\_Weile\_2017}                         & 0.10                  & 0.15                  & 0.26                  & 0.29                   & 0.28                             & 0.27                                        & 0.23                           \\
\texttt{TPMT\_HUMAN\_Matreyek\_2018}                      & 0.37                  & 0.46                  & 0.51                  & 0.51                   & 0.54                             & 0.51                                        & 0.55                           \\
\texttt{UBC9\_HUMAN\_Weile\_2017}                         & 0.24                  & 0.44                  & 0.47                  & 0.45                   & 0.48                             & 0.5                                         & 0.54                           \\
\texttt{UBE4B\_MOUSE\_Starita\_2013}                      & -0.01                 & 0.33                  & 0.33                  & 0.30                   & 0.46                             & 0.35                                        & 0.48                           \\
\texttt{YAP1\_HUMAN\_Araya\_2012}                         & 0.16                  & 0.18                  & 0.13                  & 0.19                   & 0.34                             & 0.056                                       & 0.61                           \\
\midrule
AVG fitness, for proteins under 1024 amino acids & 0.3925                & 0.4497                & 0.4547                & 0.4595                 & 0.4739                           & 0.4780                                      & 0.5197\\
\bottomrule
\end{tabular}
\label{tab:full_fitness}
\end{tiny}
\end{center}
\end{table}
